Meta Attentive Graph Convolutional Recurrent Network for Traffic Forecasting

Traffic forecasting is a fundamental problem in intelligent transportation systems. Existing traffic predictors are limited by their expressive power to model the complex spatial-temporal dependencies in traffic data, mainly due to the following limitations. Firstly, most approaches are primarily designed to model the local shared patterns, which makes them insufficient to capture the specific patterns associated with each node globally. Hence, they fail to learn each node's unique properties and diversified patterns. Secondly, most existing approaches struggle to accurately model both short- and long-term dependencies simultaneously. In this paper, we propose a novel traffic predictor, named Meta Attentive Graph Convolutional Recurrent Network (MAGCRN). MAGCRN utilizes a Graph Convolutional Recurrent Network (GCRN) as a core module to model local dependencies and improves its operation with two novel modules: 1) a Node-Specific Meta Pattern Learning (NMPL) module to capture node-specific patterns globally and 2) a Node Attention Weight Generation Module (NAWG) module to capture short- and long-term dependencies by connecting the node-specific features with the ones learned initially at each time step during GCRN operation. Experiments on six real-world traffic datasets demonstrate that NMPL and NAWG together enable MAGCRN to outperform state-of-the-art baselines on both short- and long-term predictions.

==> ref.tex <==
% \RequirePackage{filecontents}
% \begin{filecontents}{\mybibfile.bib}
@article{LinASO,
  title={A survey on internet of things: Architecture, enabling technologies, security and privacy, and applications},
  author={Lin, Jie and Yu, Wei and Zhang, Nan and Yang, Xinyu and Zhang, Hanlin and Zhao, Wei},
  journal={IEEE Internet of Things Journal},
  volume={4},
  number={5},
  pages={1125--1142},
  year={2017},
  publisher={IEEE}
}
@article{ZhangDataDrivenIT,
  title={Data-driven intelligent transportation systems: A survey},
  author={Zhang, Junping and Wang, Fei-Yue and Wang, Kunfeng and Lin, Wei-Hua and Xu, Xin and Chen, Cheng},
  journal={IEEE Transactions on Intelligent Transportation Systems},
  volume={12},
  number={4},
  pages={1624--1639},
  year={2011},
  publisher={IEEE}
}
@article{Zhu2019BigDA,
  title={Big data analytics in intelligent transportation systems: A survey},
  author={Zhu, Li and Yu, Fei Richard and Wang, Yige and Ning, Bin and Tang, Tao},
  journal={IEEE Transactions on Intelligent Transportation Systems},
  volume={20},
  number={1},
  pages={383--398},
  year={2018},
  publisher={IEEE}
}
@article{Jia2018DataDC,
  title={Data driven congestion trends prediction of urban transportation},
  author={Jia, Rui and Jiang, Pengcheng and Liu, Lei and Cui, Lizhen and Shi, Yuliang},
  journal={IEEE Internet of Things Journal},
  volume={5},
  number={2},
  pages={581--591},
  year={2017},
  publisher={IEEE}
}
@article{Kong2013UTNModelBasedTF,
  title={UTN-model-based traffic flow prediction for parallel-transportation management systems},
  author={Kong, Qing-Jie and Xu, Yanyan and Lin, Shu and Wen, Ding and Zhu, Fenghua and Liu, Yuncai},
  journal={IEEE Transactions on Intelligent Transportation Systems},
  volume={14},
  number={3},
  pages={1541--1547},
  year={2013},
  publisher={IEEE}
}
@article{Li2022DynamicGC,
  title={Dynamic graph convolutional recurrent network for traffic prediction: Benchmark and solution},
  author={Li, Fuxian and Feng, Jie and Yan, Huan and Jin, Guangyin and Yang, Fan and Sun, Funing and Jin, Depeng and Li, Yong},
  journal={ACM Transactions on Knowledge Discovery from Data},
  volume={17},
  number={1},
  pages={1--21},
  year={2023},
  publisher={ACM New York, NY}
}
@inproceedings{Li2018DiffusionCR,
  title={Diffusion Convolutional Recurrent Neural Network: Data-Driven Traffic Forecasting},
  author={Li, Yaguang and Yu, Rose and Shahabi, Cyrus and Liu, Yan},
  booktitle={International Conference on Learning Representations},
  year={2018}
}
@inproceedings{Hahypernetwork,
  title={Hypernetworks},
  author={Hu, David and Dai, Andrew and V. Le, Quoc},
  booktitle={International Conference on Learning Representations},
  year={2017}
}
@inproceedings{Balazevic2018HypernetworkKG,
  title={Hypernetwork Knowledge Graph Embeddings},
  author={Ivana Balazevic and Carl Allen and Timothy M. Hospedales},
  booktitle={International Conference on Artificial Neural Networks},
  pages={553--565},
  year={2018}
}
@inproceedings{Yu2018SpatioTemporalGC,
  title={Spatio-temporal graph convolutional networks: a deep learning framework for traffic forecasting},
  author={Yu, Bing and Yin, Haoteng and Zhu, Zhanxing},
  booktitle={Proceedings of the 27th International Joint Conference on Artificial Intelligence},
  pages={3634--3640},
  year={2018}
}
@inproceedings{Zheng2020GMANAG,
  title={Gman: A graph multi-attention network for traffic prediction},
  author={Zheng, Chuanpan and Fan, Xiaoliang and Wang, Cheng and Qi, Jianzhong},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  pages={1234--1241},
  year={2020},
  publisher={IEEE}
}
@inproceedings{Jiang2021DLTraffSA,
  title={Dl-traff: Survey and benchmark of deep learning models for urban traffic prediction},
  author={Jiang, Renhe and Yin, Du and Wang, Zhaonan and Wang, Yizhuo and Deng, Jiewen and Liu, Hangchen and Cai, Zekun and Deng, Jinliang and Song, Xuan and Shibasaki, Ryosuke},
  booktitle={Proceedings of the 30th ACM international conference on information \& knowledge management},
  pages={4515--4525},
  year={2021}
}
@article{Williams2003ModelingAF,
  title={Modeling and Forecasting Vehicular Traffic Flow as a Seasonal ARIMA Process: Theoretical Basis and Empirical Results},
  author={Billy M. Williams and Lester A. Hoel},
  journal={Journal of Transportation Engineering},
  year={2003},
  volume={129},
  pages={664-672}
}
@inproceedings{Zivot2003VectorAM,
  title={Vector Autoregressive Models for Multivariate Time Series},
  author={Eric Zivot and Jiahui Wang},
  booktitle={Modeling Financial Time Series With S-Plus},
  pages={385--429},
  year={2003}
}
@inproceedings{Drucker1996SupportVR,
  title={Support Vector Regression Machines},
  author={Harris Drucker and Christopher J. C. Burges and Linda Kaufman and Alex Smola and Vladimir Naumovich Vapnik},
  booktitle={Neural Information Processing Systems},
  pages={155--161},
  year={1997}
}
@inproceedings{Kipf2017SemiSupervisedCW,
  title={Semi-supervised classification with graph convolutional networks},
  author={Welling, Max and Kipf, Thomas N},
  booktitle={International Conference on Learning Representations},
  year={2016}
}
@inproceedings{Velickovic2018GraphAN,
  title={Graph Attention Networks},
  author={Veli{\v{c}}kovi{\'c}, Petar and Cucurull, Guillem and Casanova, Arantxa and Romero, Adriana and Li{\`o}, Pietro and Bengio, Yoshua},
  booktitle={International Conference on Learning Representations},
  year={2018}
}
@article{Hochreiter1997LongSM,
  title={Long Short-Term Memory},
  author={Sepp Hochreiter and Jurgen Schmidhuber},
  journal={Neural Computation},
  year={1997},
  volume={9},
  pages={1735-1780}
}
@article{LeCun1998GradientbasedLA,
  title={Gradient-based learning applied to document recognition},
  author={LeCun, Yann and Bottou, L{\'e}on and Bengio, Yoshua and Haffner, Patrick},
  journal={Proceedings of the IEEE},
  volume={86},
  number={11},
  pages={2278--2324},
  year={1998},
  publisher={Ieee}
}
@inproceedings{Yu2015MultiScaleCA,
  title={Multi-Scale Context Aggregation by Dilated Convolutions},
  author={Fisher Yu and Vladlen Koltun},
  booktitle={International Conference on Learning Representations},
  year={2016}
}
@inproceedings{Vaswani2017AttentionIA,
  title={Attention is All you Need},
  author={Ashish Vaswani and Noam M. Shazeer and Niki Parmar and Jakob Uszkoreit and Llion Jones and Aidan N. Gomez and Lukasz Kaiser and Illia Polosukhin},
  booktitle={Neural Information Processing Systems},
  pages={5998--6008},
  year={2017}
}
@inproceedings{Wu2019GraphWF,
  title={Graph wavenet for deep spatial-temporal graph modeling},
  author={Wu, Zonghan and Pan, Shirui and Long, Guodong and Jiang, Jing and Zhang, Chengqi},
  booktitle={Proceedings of the 28th International Joint Conference on Artificial Intelligence},
  pages={1907--1913},
  year={2019}
}
@inproceedings{Wang2020TrafficFP,
  title={Traffic flow prediction via spatial temporal graph neural network},
  author={Wang, Xiaoyang and Ma, Yao and Wang, Yiqi and Jin, Wei and Wang, Xin and Tang, Jiliang and Jia, Caiyan and Yu, Jian},
  booktitle={Proceedings of The Web Conference},
  pages={1082--1092},
  year={2020}
}
@inproceedings{Wu2020ConnectingTD,
  title={Connecting the dots: Multivariate time series forecasting with graph neural networks},
  author={Wu, Zonghan and Pan, Shirui and Long, Guodong and Jiang, Jing and Chang, Xiaojun and Zhang, Chengqi},
  booktitle={Proceedings of the 26th ACM SIGKDD International Conference on Knowledge Discovery and Data Mining},
  pages={753--763},
  year={2020}
}
@article{Bai2020AdaptiveGC,
  title={Adaptive graph convolutional recurrent network for traffic forecasting},
  author={Bai, Lei and Yao, Lina and Li, Can and Wang, Xianzhi and Wang, Can},
  journal={Advances in Neural Information Processing Systems},
  pages={17804--17815},
  year={2020}
}
@inproceedings{Guo2019AttentionBS,
  title={Attention based spatial-temporal graph convolutional networks for traffic flow forecasting},
  author={Guo, Shengnan and Lin, Youfang and Feng, Ning and Song, Chao and Wan, Huaiyu},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  pages={922--929},
  year={2019}
}
@inproceedings{Pascanu2012OnTD,
  title={On the difficulty of training recurrent neural networks},
  author={Razvan Pascanu and Tomas Mikolov and Yoshua Bengio},
  booktitle={International Conference on Machine Learning},
  pages={1310--1318},
  year={2013}
}
@article{Bengio1994LearningLD,
  title={Learning long-term dependencies with gradient descent is difficult},
  author={Yoshua Bengio and Patrice Y. Simard and Paolo Frasconi},
  journal={IEEE Transactions on Neural Networks},
  volume={5},
  number={2},
  pages={157-66},
  year={1994}
}
@inproceedings{huang2019dsanet,
  title={Dsanet: Dual self-attention network for multivariate time series forecasting},
  author={Huang, Siteng and Wang, Donglin and Wu, Xuehan and Tang, Ao},
  booktitle={Proceedings of the 28th ACM international conference on information and knowledge management},
  pages={2129--2132},
  year={2019}
}
@inproceedings{lan2022dstagnn,
  title={Dstagnn: Dynamic spatial-temporal aware graph neural network for traffic flow forecasting},
  author={Lan, Shiyong and Ma, Yitong and Huang, Weikang and Wang, Wenwu and Yang, Hongyu and Li, Pyang},
  booktitle={International Conference on Machine Learning},
  pages={11906--11917},
  year={2022},
  organization={PMLR}
}
@inproceedings{Huang2020LSGCNLS,
  title={LSGCN: long short-term traffic prediction with graph convolutional networks},
  author={Huang, Rongzhou and Huang, Chuyin and Liu, Yubao and Dai, Genan and Kong, Weiyang},
  booktitle={Proceedings of the 29th International Joint Conferences on Artificial Intelligence},
  pages={2355--2361},
  year={2021}
}
@inproceedings{chen2021z,
  title={Z-GCNETs: Time zigzags at graph convolutional networks for time series forecasting},
  author={Chen, Yuzhou and Segovia, Ignacio and Gel, Yulia R},
  booktitle={International Conference on Machine Learning},
  pages={1684--1694},
  year={2021},
  organization={PMLR}
}
@inproceedings{Cho2014LearningPR,
  title={Learning Phrase Representations using RNN Encoder--Decoder for Statistical Machine Translation},
  author={Cho, Kyunghyun and van Merri{\"e}nboer, Bart and Gul{\c{c}}ehre, {\c{C}}a{\u{g}}lar and Bahdanau, Dzmitry and Bougares, Fethi and Schwenk, Holger and Bengio, Yoshua},
  booktitle={Proceedings of the 2014 Conference on Empirical Methods in Natural Language Processing (EMNLP)},
  pages={1724--1734},
  year={2014}
}

@article{Zhao2020TGCNAT,
  title={T-gcn: A temporal graph convolutional network for traffic prediction},
  author={Zhao, Ling and Song, Yujiao and Zhang, Chao and Liu, Yu and Wang, Pu and Lin, Tao and Deng, Min and Li, Haifeng},
  journal={IEEE Transactions on Intelligent Transportation Systems},
  volume={21},
  number={9},
  pages={3848--3858},
  year={2019},
  publisher={IEEE}
}
@inproceedings{Cohen2016GroupEC,
  title={Group equivariant convolutional networks},
  author={Cohen, Taco and Welling, Max},
  booktitle={International Conference on Machine Learning},
  pages={2990--2999},
  year={2016}
}
@inproceedings{Nguyen2018ANE,
  title={A Novel Embedding Model for Knowledge Base Completion Based on Convolutional Neural Network},
  author={Nguyen, Tu Dinh and Nguyen, Dat Quoc and Phung, Dinh and others},
  booktitle={Proceedings of the 2018 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies, Volume 2 (Short Papers)},
  pages={327--333},
  year={2018}
}
@inproceedings{Kingma2015AdamAM,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  booktitle={International Conference on Learning Representations},
  year={2015}
}
@inproceedings{Snyder2019STREETSAN,
  title={STREETS: a novel camera network dataset for traffic flow},
  author={Snyder, Corey and Do, Minh N},
  booktitle={Proceedings of the 33rd International Conference on Neural Information Processing Systems},
  pages={10242--10253},
  year={2019}
}
@article{Lim2019TemporalFT,
  title={Temporal Fusion Transformers for Interpretable Multi-horizon Time Series Forecasting},
  author={Bryan Lim and Sercan {\"O}. Arik and Nicolas Loeff and Tomas Pfister},
  journal={International Journal of Forecasting},
  volume={37},
  pages={1748--1764},
  year={2021},
  publisher={Elsevier}
}
@inproceedings{Bai2019STG2SeqSG,
  title={STG2seq: spatial-temporal graph to sequence model for multi-step passenger demand forecasting},
  author={Bai, Lei and Yao, Lina and Kanhere, Salil S and Wang, Xianzhi and Sheng, Quan Z},
  booktitle={Proceedings of the 28th International Joint Conference on Artificial Intelligence},
  pages={1981--1987},
  year={2019}
}
@inproceedings{Bai2019PassengerDF,
  title={Passenger demand forecasting with multi-task convolutional recurrent neural networks},
  author={Bai, Lei and Yao, Lina and Kanhere, Salil S and Yang, Zheng and Chu, Jing and Wang, Xianzhi},
  booktitle={Pacific-Asia Conference on Knowledge Discovery and Data Mining},
  pages={29--42},
  year={2019}
}
@inproceedings{Tang2020JointMO,
  title={Joint modeling of local and global temporal dynamics for multivariate time series forecasting with missing values},
  author={Tang, Xianfeng and Yao, Huaxiu and Sun, Yiwei and Aggarwal, Charu and Mitra, Prasenjit and Wang, Suhang},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  pages={5956--5963},
  year={2020}
}
@inproceedings{Yao2018DeepMS,
  title={Deep multi-view spatial-temporal network for taxi demand prediction},
  author={Yao, Huaxiu and Wu, Fei and Ke, Jintao and Tang, Xianfeng and Jia, Yitian and Lu, Siyu and Gong, Pinghua and Ye, Jieping and Li, Zhenhui},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  pages={2588--2595},
  year={2018}
}
@article{Flunkert2020DeepARPF,
  title={DeepAR: Probabilistic forecasting with autoregressive recurrent networks},
  author={Salinas, David and Flunkert, Valentin and Gasthaus, Jan and Januschowski, Tim},
  journal={International Journal of Forecasting},
  volume={36},
  number={3},
  pages={1181--1191},
  year={2020},
  publisher={Elsevier}
}
@inproceedings{Song2020SpatialTemporalSG,
  title={Spatial-temporal synchronous graph convolutional networks: A new framework for spatial-temporal network data forecasting},
  author={Song, Chao and Lin, Youfang and Guo, Shengnan and Wan, Huaiyu},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  pages={914--921},
  year={2020}
}
@inproceedings{li2021spatial,
  title={Spatial-temporal fusion graph neural networks for traffic flow forecasting},
  author={Li, Mengzhang and Zhu, Zhanxing},
  booktitle={Proceedings of the AAAI conference on artificial intelligence},
  volume={35},
  number={5},
  pages={4189--4196},
  year={2021}
}
@inproceedings{Pan2019UrbanTP,
  title={Urban traffic prediction from spatio-temporal data using deep meta learning},
  author={Pan, Zheyi and Liang, Yuxuan and Wang, Weifeng and Yu, Yong and Zheng, Yu and Zhang, Junbo},
  booktitle={Proceedings of the 25th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining},
  pages={1720--1730},
  year={2019}
}
@inproceedings{Liao2018DeepSL,
  title={Deep sequence learning with auxiliary information for traffic prediction},
  author={Liao, Binbing and Zhang, Jingqing and Wu, Chao and McIlwraith, Douglas and Chen, Tong and Yang, Shengwen and Guo, Yike and Wu, Fei},
  booktitle={Proceedings of the 24th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining},
  pages={537--546},
  year={2018}
}
@inproceedings{Lv2018LCRNNAD,
  title={LC-RNN: a deep learning model for traffic speed prediction},
  author={Lv, Zhongjian and Xu, Jiajie and Zheng, Kai and Yin, Hongzhi and Zhao, Pengpeng and Zhou, Xiaofang},
  booktitle={Proceedings of the 27th International Joint Conference on Artificial Intelligence},
  pages={3470--3476},
  year={2018}
}
@article{Wang2019TrafficSP,
  title={Traffic speed prediction for urban transportation network: A path based deep learning approach},
  author={Wang, Jiawei and Chen, Ruixiang and He, Zhaocheng},
  journal={Transportation Research Part C: Emerging Technologies},
  volume={100},
  pages={372--385},
  year={2019},
  publisher={Elsevier}
}
@inproceedings{Diao2019DynamicSG,
  title={Dynamic spatial-temporal graph convolutional neural networks for traffic forecasting},
  author={Diao, Zulong and Wang, Xin and Zhang, Dafang and Liu, Yingru and Xie, Kun and He, Shaoyao},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  pages={890--897},
  year={2019}
}
@article{Guo2019DeepS3,
  title={Deep spatial--temporal 3D convolutional neural networks for traffic data forecasting},
  author={Guo, Shengnan and Lin, Youfang and Li, Shijie and Chen, Zhaoming and Wan, Huaiyu},
  journal={IEEE Transactions on Intelligent Transportation Systems},
  volume={20},
  number={10},
  pages={3913--3926},
  year={2019},
  publisher={IEEE}
}
@article{Yu2022GraphCF,
  title={Graph Construction for Traffic Prediction: A Data-Driven Approach},
  author={James J. Q. Yu},
  journal={IEEE Transactions on Intelligent Transportation Systems},
  volume={23},
  number={10},
  pages={15015-15027},
  year={2022},
  publisher={IEEE}
}
@article{Yu2021LongTermUT,
  title={Long-Term Urban Traffic Speed Prediction With Deep Learning on Graphs},
  author={James J. Q. Yu and Christos Markos and Shiyao Zhang},
  journal={IEEE Transactions on Intelligent Transportation Systems},
  volume={23},
  number={7},
  pages={7359-7370},
  year={2021},
  publisher={IEEE}
}
@article{tkdeYujames,
  author={Yu, James J.Q.},
  journal={IEEE Transactions on Knowledge and Data Engineering}, 
  title={Citywide Estimation of Travel Time Distributions with Bayesian Deep Graph Learning}, 
  year={2021},
  volume={},
  number={},
  pages={1-1},
  doi={10.1109/TKDE.2021.3117986}}

@article{tkdeGuo,
  author={Guo, Shengnan and Lin, Youfang and Wan, Huaiyu and Li, Xiucheng and Cong, Gao},
  journal={IEEE Transactions on Knowledge and Data Engineering}, 
  title={Learning Dynamics and Heterogeneity of Spatial-Temporal Graph Data for Traffic Forecasting}, 
  year={2022},
  volume={34},
  number={11},
  pages={5415-5428},
  doi={10.1109/TKDE.2021.3056502}}

@inproceedings{vanwavenet,
  title={WaveNet: A Generative Model for Raw Audio},
  author={van den Oord, A{\"a}ron and Dieleman, Sander and Zen, Heiga and Simonyan, Karen and Vinyals, Oriol and Graves, Alex and Kalchbrenner, Nal and Senior, Andrew and Kavukcuoglu, Koray},
  booktitle={9th ISCA Speech Synthesis Workshop},
  pages={125--125}
}

@article{bai2018empirical,
  title={An empirical evaluation of generic convolutional and recurrent networks for sequence modeling},
  author={Bai, Shaojie and Kolter, J Zico and Koltun, Vladlen},
  journal={arXiv preprint arXiv:1803.01271},
  year={2018}
}

@article{tkdeBaggag,
  author={Baggag, Abdelkader and Abbar, Sofiane and Sharma, Ankit and Zanouda, Tahar and Al-Homaid, Abdulaziz and Mohan, Abhiraj and Srivastava, Jaideep},
  journal={IEEE Transactions on Knowledge and Data Engineering}, 
  title={Learning Spatiotemporal Latent Factors of Traffic via Regularized Tensor Factorization: Imputing Missing Values and Forecasting}, 
  year={2021},
  volume={33},
  number={6},
  pages={2573-2587},
  doi={10.1109/TKDE.2019.2954868}}

@article{tkdeJin,
  author={Jin, Ming and Zheng, Yu and Li, Yuan-Fang and Chen, Siheng and Yang, Bin and Pan, Shirui},
  journal={IEEE Transactions on Knowledge and Data Engineering}, 
  title={Multivariate Time Series Forecasting with Dynamic Graph Neural ODEs}, 
  year={2022},
  volume={},
  number={},
  pages={1-14},
  doi={10.1109/TKDE.2022.3221989}}
% \end{filecontents}
